RoCourseNet: Distributionally Robust Training of a Prediction Aware Recourse Model

Counterfactual (CF) explanations for machine learning (ML) models are preferred by end-users, as they explain the predictions of ML models by providing a recourse (or contrastive) case to individuals who are adversely impacted by predicted outcomes. Existing CF explanation methods generate recourses under the assumption that the underlying target ML model remains stationary over time. However, due to commonly occurring distributional shifts in training data, ML models constantly get updated in practice, which might render previously generated recourses invalid and diminish end-users trust in our algorithmic framework. To address this problem, we propose RoCourseNet, a training framework that jointly optimizes predictions and recourses that are robust to future data shifts. This work contains four key contributions: (1) We formulate the robust recourse generation problem as a tri-level optimization problem which consists of two sub-problems: (i) a bi-level problem that finds the worst-case adversarial shift in the training data, and (ii) an outer minimization problem to generate robust recourses against this worst-case shift. (2) We leverage adversarial training to solve this tri-level optimization problem by: (i) proposing a novel virtual data shift (VDS) algorithm to find worst-case shifted ML models via explicitly considering the worst-case data shift in the training dataset, and (ii) a block-wise coordinate descent procedure to optimize for prediction and corresponding robust recourses. (3) We evaluate RoCourseNet's performance on three real-world datasets, and show that RoCourseNet consistently achieves more than 96% robust validity and outperforms state-of-the-art baselines by at least 10% in generating robust CF explanations. (4) Finally, we generalize the RoCourseNet framework to accommodate any parametric post-hoc methods for improving robust validity.

==> sections/03_preliminary.tex <==
We now discuss the counterfactual explanation (or recourse) problem, and describe the CounterNet architecture \cite{guo2021counternet}, which we use as a building block for RoCourseNet. For ease of exposition, we focus on binary classification problems, but our techniques can be adapted to multi-class settings\footnote{See appendix for detailed discussions about extensions to multi-class settings.}.
Note that we use $\mathcal{L}(\cdot,\cdot)$ to represent the mean squared error (MSE) loss function (following \citep{guo2021counternet}).

\textbf{Counterfactual Explanations.} 
Given an input instance $x$ and an ML model $f(\cdot; \theta)$ as input, a counterfactual explanation method finds a CF example (or recourse) $\cf$ which receives an opposite prediction from the ML model (i.e., $f(\cf; \theta) =  1-f(x; \theta)$), while ensuring a low cost of change (i.e., the ``distance" between $x$ and $\cf$ is low). Let $c(x, \cf)$ denote the cost of change (e.g., $L_1$-norm distance function) from ${x}$ to $\cf$. Then, most prior techniques \citep{wachter2017counterfactual,mothilal2020explaining,ustun2019actionable} generate CF explanations $\cf$ by solving the following optimization problem separately for each input instance $x$:
\begin{equation}
    \label{eq:cf}
    \cf = \operatorname{argmin}_{\cf} \ \mathcal{L}\big(f(\cf; \theta), 1 - f(x; \theta)\big) + \lambda \cdot c(x, \cf)
\end{equation}
The first part of Eq.~\ref{eq:cf} maximizes the validity to ensure that the generated recourse $\cf$ gets an opposite prediction to $x$.
% between the prediction received on data points $x$ and $\cf$, which ensures that the generated recourse $\cf$ gets an opposite prediction from the predictive model. 
The second part of Eq. \ref{eq:cf} minimizes the cost of change (or distance) between $x$ and $\cf$. Finally, $\lambda$ balances the trades-off between the two objective terms.



\textbf{CounterNet.} Unlike post-hoc methods described above (Eq. \ref{eq:cf}), CounterNet \citep{guo2021counternet} is an end-to-end framework which combines predictive model training and counterfactual explanation generation into a single optimization pipeline. At a high level, given an instance $x$ as input, CounterNet produces two outputs: (i) the predictive label $f(x; \theta_f)$ of the input instance $x$, where $\theta_f = \{\theta_h,\theta_m\}$ in Figure~\ref{fig:architecture}; and (ii) the corresponding recourse $\cf$ for instance $x$. CounterNet has three learning objectives:
\begin{equation}
    \label{eq:object}
    \operatorname*{argmin}_{\mathbf{\theta}=\{\theta_h, \theta_m, \theta_g\}} 
    \mathbb{E}_{\left(x, y\right) \sim D}
    \Big[ 
    \lambda_1 \cdot \underbrace{\mathcal{L}\Big(y, f\left(x; \theta_f\right)\Big)}_{\text{Prediction Loss (${L}_1$)}} + 
    \lambda_2 \cdot \underbrace{\mathcal{L}\Big(f(\cf; \theta_f), 1 - f(x; \theta_f)\Big)}_{\text{Validity Loss (${L}_2$)}} + 
    \lambda_3 \cdot \!\!\! \underbrace{\mathcal{L}\Big(x, \cf\Big)}_{\text{Proximity Loss (${L}_3$)}} \!\!\!
    \Big]
\end{equation}
where ($\lambda_1$, $\lambda_2$, $\lambda_3$) balance the three loss components. The prediction loss $L_1$ maximizes predictive accuracy. Similarly, the validity loss $L_2$ maximizes validity by ensuring that predictions on $\cf$ and $x$ differs. Finally, the proximity loss $L_3$ minimizes the cost of change required to go from $x$ to $\cf$. %Furthermore, all loss functions $\mathcal{L}(\cdot)$ in Eq.~\ref{eq:object} denote the mean squared error (MSE).
% The prediction loss $\mathcal{L}_1$ denotes the mean squared error (MSE) between the actual and the predicted labels ($y$ and $f(x; \theta_f)$ on instance $x$, respectively), which aims to maximize predictive accuracy. Similarly, the validity loss $\mathcal{L}_2$ denotes the MSE between the prediction on instance $x$ (i.e., $f(x; \theta_f)$), and the opposite of the prediction received by the corresponding CF example $\cf$ (i.e., $1 - f(\cf; \theta_f)$). Intuitively, minimizing $\mathcal{L}_2$ maximizes the validity of the generated CF example $\cf$ by ensuring that the predictions on $\cf$ and $x$ are different. Finally, the proximity loss $\mathcal{L}_3$ denotes the MSE between $x$ and $\cf$, which aims to minimize the cost of change required to go from $x$ to $\cf$.

To optimize Eq.~\ref{eq:object}, \citet{guo2021counternet} proposed a block-wise coordinate descent approach. Specifically, for each mini-batch, CounterNet's parameters are updated twice: it first computes $\theta' = \theta - \nabla_\theta (\lambda_1 \cdot {L}_1)$, and for the second update, it computes $\theta'' = \theta' - \nabla_{\theta'} (\lambda_2 \cdot {L}_2 + \lambda_3 \cdot {L}_3)$ (in Eq~\ref{eq:object}). 
This coordinate descent procedure ensures that CounterNet achieves state-of-the-art results on static datasets.%, e.g., it maintains more than 98\% validity and has the lowest proximity across four out of six benchmarked datasets. %A key reason for CounterNet's superior performance stems from its design on its model prediction and CF explanation deriving from a shared component (i.e., the encoder $h(\cdot)$ in Fig.~\ref{fig:architecture}). 


Unfortunately, despite promising performance on static datasets, CounterNet is not explicitly designed for scenarios where the predictive models get updated due to shifts in the data distribution.
% (e.g., when CounterNet is evaluated on a held-out test dataset i.i.d. to the training dataset), 
% the CF explanations generated by CounterNet are not robust to model shifts induced by shifts in the data distribution. 
As our experimental evaluation suggests, CounterNet's validity score degrades by $\sim$25\% when the predictive model is updated with new available data (see Section~\ref{sec:experiment}), which reveals the limitations of CounterNet as it fails to generate CF examples robust to model shifts. 
% For example, our experimental evaluation shows that the validity of recourses generated by CounterNet degrades by $\sim$25\% when the predictive model is updated with new available data (see Section~\ref{sec:experiment}). This illustrates that CounterNet is unsuitable for recourse generation in real-world domains where frequent updates to the data distribution are common (e.g., when new data is periodically made available, leading to a periodic shift in the model). 
In this paper, we propose an approach built upon CounterNet, which optimizes for robust recourse generation against data shifts.

%Next, we discuss the proposed approach to improve the robustness of CounterNet against the model shift.


%We show that the regular CounterNet drops $~25\%$ validity when the model is updated by new data sources (see Section~\ref{sec:experiment}), which illustrates the needs for improving the robustness of the CounterNet under distribution shift. Next, we discuss the proposed approach to improve the robustness of CounterNet against the model shift.


\begin{figure}[t!]
\centering
\includegraphics[width=0.9\linewidth]{figs/architecture-1.pdf}
\caption{The architecture of CounterNet, the building block of RoCourseNet (\citet{guo2021counternet}).}
\label{fig:architecture}
\end{figure}
% \vspace{-10pt}


==> sections/07_statement.tex <==
\textbf{Ethics Statement.}
% Although CounterNet is suitable for real-time deployment given its superior performance in its highly aligned CF explanations and speed, one must be aware of the possible negative impacts of its CF explanations to human end-users. It is important to ensure that generated CF examples do not amplify or provide support to the narratives resulting from pre-existing race-based and gender-based societal inequities (among others).
% As we stated in Section~\ref{sec:conclusion}, one short-term workaround is to have humans in the loop. We can provide CounterNet’s explanations as a decision-aid to a well-trained human official, who is in charge of communicating the decisions of ML models to human end-users in a respectful and humane manner. In the long-run, further qualitative and quantitative studies are needed to understand the social impacts of CounterNet.
RoCoursenet takes into account of potential model shift in the real-world deployment. However, before deploying RoCourseNet to a real-world system, one must be aware of the possibility for RoCourseNet to reinforce pre-existing societal prejudices among end users. A temporary workaround is to have trained human operators to communicate the CF explanations in a respectful manner. In the long term, more quantitative and qualitative research will be required to fully understand RoCourseNet's societal impact.



\textbf{Reproducibility Statement.}
We release the code through an anonymous repository in supporting the reproduction of this work ((\url{https://github.com/bkghz-orange-blue/counternet_adv}). 
In this anonymous repository, we also offer the dataset that was utilized for this paper's evaluation. We also include the options for hyperparameters in the appendix~\ref{sec:app-implementation}.
Appendix~\ref{sec:app-implementation} contains a thorough description of our experimental implementation.

% It is important that the work published in ICLR is reproducible. Authors are strongly encouraged to include a paragraph-long Reproducibility Statement at the end of the main text (before references) to discuss the efforts that have been made to ensure reproducibility. This paragraph should not itself describe details needed for reproducing the results, but rather reference the parts of the main paper, appendix, and supplemental materials that will help with reproducibility. For example, for novel models or algorithms, a link to a anonymous downloadable source code can be submitted as supplementary materials; for theoretical results, clear explanations of any assumptions and a complete proof of the claims can be included in the appendix; for any datasets used in the experiments, a complete description of the data processing steps can be provided in the supplementary materials. Each of the above are examples of things that can be referenced in the reproducibility statement. This optional reproducibility statement will not count toward the page limit, but should not be more than 1 page.


